Efficacy of EPSS in High Severity CVEs found in KEV

The Exploit Prediction Scoring System (EPSS) is designed to assess the probability of a vulnerability being exploited in the next 30 days relative to other vulnerabilities. The latest version, based on a research paper published in arXiv, assists defenders in deciding which vulnerabilities to prioritize for remediation. This study evaluates EPSS's ability to predict exploitation before vulnerabilities are actively compromised, focusing on high severity CVEs that are known to have been exploited and included in the CISA KEV catalog. By analyzing EPSS score history, the availability and simplicity of exploits, the system's purpose, its value as a target for Threat Actors (TAs), this paper examines EPSS's potential and identifies areas for improvement.

==> CVE/CVE-2024-21893.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%d NOT USING THIS ONE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CVE-2024-21893 (\textit{remote access technology})}
%%%%%%%%%%INSERT GRAPH OF PROBABILITIES HERE CVE-2024-21893%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ivanti Connect Secure (ICS, formerly known as Pulse Connect Secure), Ivanti Policy Secure, and Ivanti Neurons contain a server-side request forgery (SSRF) vulnerability in the SAML component that allows an attacker to access certain restricted resources without authentication. A detailed analysis explaining the vulnerability was published on 2/2/2024 \cite{IvantiConnectDetails}. A public exploit was available a few days after the CVE was published \cite{IvantiConnectExploit}
A Metasploit module was made available on 2/22/2024.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\columnwidth, 
%bb=0 0 600 400
]{CVE/images/CVE-2024-21893EPSSScore.eps}
    \caption{CVE-2024-21893 EPSS Details}
    \label{fig:CVE-2024-21893}
\end{figure}

\begin{comment}

EPSS DATA:
\input{JSON/CVE-2024-21893.json}

PUBLIC EXPLOIT AVAILABLE DATE:  02/02/2024
\cite{@misc{IvantiConnectExploit,
  author  = {h4x0r-dz},
  title   = {CVE-2024-21893.py},
  day     = {02},
  month   = {02},
  year    = {2024},
  url     = {https://github.com/h4x0r-dz/CVE-2024-21893.py},
  note = {Accessed: 2024-07-07}
}}

\cite{@article{IvantiConnectDetails,
  title   = {CVE-2024-21893: Rapid7 Analysis},
  author  = {Caitlin Condon},
  journal = {AttackerKB},
  day     = {02},
  month   = {02},
  year    = {2024},
  url     = {https://attackerkb.com/topics/FGlK1TVnB2/cve-2024-21893/rapid7-analysis}
}}

RANSOMWARE: n/a
\cite {}

CVE DATE: 2024-01-31
KEV DATE: 2024-01-31
\end{comment}
